High-Order Continuous Geometrical Validity

We propose a conservative algorithm to test the geometrical validity of simplicial (triangles, tetrahedra), tensor product (quadrilaterals, hexahedra), and mixed (prisms) elements of arbitrary polynomial order as they deform over a piecewise-linear trajectory. Our algorithm uses a combination of adaptive B\'ezier refinement and bisection search to determine if, when, and where the Jacobian determinant of an element's polynomial geometric map becomes negative in the transition from one configuration to another. Unlike previous approaches, our method preserves its properties also when implemented using floating point arithmetic: This feature comes at a small additional runtime cost compared to existing inexact methods, making it a drop-in replacement for current validity tests, while providing superior robustness and generality. To prove the practical effectiveness of our algorithm, we demonstrate its use in a high-order Incremental Potential Contact (IPC) elastodynamic simulator, and we experimentally show that it prevents invalid, simulation-breaking configurations that would otherwise occur using inexact methods, without the need for manual parameter tuning.

==> algorithms-old.tex <==
\EP{All algorithms should be moved to the previous section and described in terms of the generic inclusion function.}

\begin{algorithm}[htb]
\caption{Recursive Bézier refinement}
\label{alg:bezierRefine}
\begin{algorithmic}[1]
\Require{Polynomial as a vector $b$ of Bézier coefficients; current and maximum recursion depths $l$ and $L$.}
\Ensure{(Sub)element validity as one of \EValid, \EInvalid, \EUncertain}

\Function{Subdivide}{$b, l$}
	\If {$l>L$}
		\State \Return \EUncertain
	\EndIf
	\For{$q=1,\dots,Q$}
		\State $b^q\gets \transition{\bezpoly}{\bezpoly}^q b$
		\For{$c\in\cornerset_\sigma^m$}
			\If{$b^q_c \leq 0$}
				\State \Return \EInvalid
			\EndIf
		\EndFor
	\EndFor

	\For{$q=1,\dots,Q$}
		\For{$i\in \indexset_\sigma(m)$}
			\If{$b^q_i \leq 0$}
				\State $u\gets$\Call{Subdivide}{$b^q,l+1$}
				\If{$u \neq \EValid$}
					\State \Return $u$
				\EndIf
			\EndIf
		\EndFor
	\EndFor
	\State \Return \EValid
\EndFunction

\end{algorithmic}
\end{algorithm}

\begin{algorithm}[htb]
\caption{Robust positivity check with Bézier refinement}
\label{alg:bezierStatic}
\begin{algorithmic}[1]
	\Require{Order $m$ polynomial $f$ on reference element $\sigma$; maximum recursion level $L$.}
	\Ensure{One of \EValid, \EInvalid, \EUncertain}

	\ForAll{$i \in \indexset_\sigma(m)$}
		\State $f^\lagpoly_i \gets f(\gamma_i)$
		\If{$f^\lagpoly_i \leq 0$}
			\State \Return \EInvalid
		\EndIf
	\EndFor
	\State $f^\bezpoly \gets \transition{\lagpoly}{\bezpoly} f^\lagpoly$
	\If{$\exists i \in \indexset_\sigma(m) : f^\bezpoly_i \leq 0$}
		\State \Return \Call{Subdivide}{$f^\bezpoly, 1$}
	\Else \State \Return \EValid
	\EndIf
\end{algorithmic}
\end{algorithm}





==> bisection.tex <==
\section{The bisection method}
\FS{not updated yet}

The bisection method (Algorithm \ref{alg:bisection}, and Figure \ref{fig:bisection}) is an adaptation of the robust root-finding algorithm for continuous collision detection presented by Wang et al. \cite{wang_large-scale_2021}. 
Although we only use this algorithm to check the positivity of Jacobian determinants, our method is general and can be used to test the positivity of any polynomial on any reference element (as defined in Section \ref{sec:formulation}).

Let $\intset{\reals}$ denote the set of real intervals.

\begin{definition}[Minimum inclusion function]
	Given $f:\reals^n\to\reals$, a function $\minclusion{f}:\intset{\reals}^n\to\intset{\reals}$ is a minimum inclusion function for $f$ if, for all $I\in\intset{\reals}^n$, we have $\min{f(I)}\in \minclusion{f}(I)$.
\end{definition}
Compare this definition to the one for the usual \emph{inclusion functions}: an inclusion function $\inclusion{f}$ produces a conservative estimate the range of $f$ in an axis-aligned box $I\in\intset{\reals}^n$; a minimum inclusion function $\minclusion{f}$ produces a conservative estimate of the minimum of $f$ in $I$. All inclusion functions for $f$ are also minimum inclusion functions for $f$.

\begin{figure}[t]
	\centering
	\input{bisectionChart.tex}
	\caption{The bisection algorithm on triangular elements.}
	\label{fig:bisection}
\end{figure}

We explore the domain $\sigma_s$ of $f$ looking for negative values, with the aid of the minimum inclusion function $\minclusion{f}$: if we find a negative value, the element is invalid; otherwise, if we explore the whole domain without finding any negative value, the element is valid.
The algorithm works as follows (Algorithm \ref{alg:bisection} and Figure \ref{fig:bisection}).
First, $\minclusion{f}$ is evaluated at $[0,1]^n$.
If the resulting interval is entirely negative, then we know that $f$ is negative in the whole box, so the element is invalid; likewise, if the interval is entirely positive, then we know it is valid: in both cases, we stop and return the corresponding answer. 
Otherwise, the interval contains zero and the element must be investigated further. 
In this case, we push the box into a data structure $S$ that supports push and pop operations (e.g., a stack or a priority queue); then we pop elements from the queue until this becomes empty and we process each box by splitting it into $2^n$ equal sub-boxes and evaluating the inclusion function in each of them.
Because of the definition of domain $\sigma_s$ of $f$ in Sec.\ref{sec:formulation}, checking for the intersection between a box and $\sigma_s$ is as simple as testing that the box corner with the smallest coordinates falls within $\sigma_s$.
If a sub-box does not intersect the domain, it needs not be investigated. 
Otherwise, if $\minclusion{f}$ is entirely negative in a sub-box, we conclude that the element is invalid; if $\minclusion{f}$ is entirely positive then that box needs not to be investigated further; finally, if $\minclusion{f}$ still contains zero, we push the sub-box into $S$ and continue. 
When $S$ becomes empty, then $f$ is positive in the whole domain and the element is valid.

We set a threshold to the maximum number of iterations, which is directly proportional to the maximum allowed running time per element, as each iteration involves the same operations. 
If we reach that threshold without finding any totally negative interval and without emptying $S$, then we return $\EUncertain$. 
Of course, our goal is to make the number of undecidable elements as small as possible. In practice, elements for which validity cannot be determined can be conservatively treated as invalid.


The criterion for extracting elements from $S$ sets the policy in which we explore the domain of $f$. 
We investigate this further in \ref{sec:traversal}.


\input{bisectionAlgorithm.tex}

\subsection{Conservative estimate of largest valid time step}
In Section \ref{sec:timedep} we explained how our formulation naturally generalizes to time-dependent validity checks.
However, when doing finite element simulation, one typically wants to find the largest possible time step $t^*\in[0,1]$ such that no element inversions occur in the transition from one frame to the next.
Our bisection algorithm can be adapted to produce a conservative estimate of $t^*$, as shown in Algorithm \ref{alg:bisectionTime}.

\FS{Maybe needs more explanation?}

\input{bisectionTimeAlgorithm.tex}


\subsection{Choosing the minimum inclusion function}
\subsubsection{Inclusion with interval arithmetic}
Inclusion functions can be computed with \emph{interval arithmetic}. It consists of a set of operations defined on the set of real intervals $\intset{\reals}$ such that if $x\in I_x \in \intset{\reals}$ and $y\in I_y \in \intset{\reals}$, then $(x*y) \in I_x * I_y$, where $*$ in the right hand side is the interval version of the operation.

Since we are dealing with polynomials, we only need the following operations:
\begin{gather}
	-[\intlo{x}, \inthi{x}] = [-\inthi{x}, -\intlo{x}] \\
	[\intlo{x}, \inthi{x}] + [\intlo{y}, \inthi{y}] =
	[\intlo{x} + \intlo{y}, \inthi{x} + \inthi{y}] \\
	[\intlo{x}, \inthi{x}] [\intlo{y}, \inthi{y}] =
	[\min(\intlo{x}\intlo{y},\intlo{x}\inthi{y},\inthi{x}\intlo{y},\inthi{x}\inthi{y}),
	\max(\intlo{x}\intlo{y},\intlo{x}\inthi{y},\inthi{x}\intlo{y},\inthi{x}\inthi{y})] \\
	[\intlo{x}, \inthi{x}]\pm r = [\intlo{x}\pm r, \inthi{x}\pm r] \quad \forall r \in \reals \\
	r [\intlo{x}, \inthi{x}] = [r \intlo{x}, r \inthi{x}] \quad \forall r\geq 0 \in \reals.
\end{gather}
By replacing all real operations with the above, we obtain a conservative estimate for the range of the function. Since any inclusion function is also a minimum inclusion function, we have a simple way of constructing $\minclusion{f}$.

Another way to view the problem in the context of multi-interval subdivision is as follows. Consider $I\in\intset{{\reals_{\geq 0}}}^n$; call $v_{\min}\in I$ the point with the smallest possible value in each coordinate (i.e. the corner that is closest to the origin) and $v_{\max}\in I$ the point with the greatest possible value in each coordinate (i.e. the corner that is farthest from the origin). The polynomial $f$ for which we are checking positivity can be written as $f_+-f_-$, where $f_+$ and $f_-$ have only positive coefficients; it is obvious that $f_+$ and $f_-$ attain their minimum and maximum in $v_{\min}$ and $v_{\max}$, respectively. The inclusion function computed with interval arithmetic returns exactly the interval $[f_+(v_{\min})-f_-(v_{\max}),f_+(v_{\max})-f_-(v_{\min})]$, which always contains the range of the function.


\subsubsection{Minimum inclusion functions}
Given an inclusion function $\inclusion{f}$, a general construction for a minimum inclusion function $\minclusion{f}$ is to replace the upper bound of $\inclusion{f}(I)$ with $\min{f(W_I)}$, where $W_I$ is any finite subset of $I$.
Regardless of the choice of $W_I$, we will get an upper bound that is at least as good as the one provided by $\inclusion{f}$.
In practice, a good heuristic for $W_I$ may allow for faster convergence.

\FS{This is the idea suggested by Daniele.}
One such heuristic is to perform a single Newton iteration starting from any internal point $\xi$ of $I$, such as the average of all box vertices that lie in the reference element $\sigma_s$. For the Newton iteration we precompute the gradient and Hessian of the polynomial $f$, and then use $W_I=\{\hat{\xi}\}$, where $\hat{\xi}=\xi-H_f^{-1}(\xi)\nabla f(\xi)$.


\subsection{Robustness with respect to floating point operations}
We explained the use of interval arithmetic as a way to automatically compute inclusion functions, but computations on intervals can be used to deal with floating point approximation error as well. For this purpose we introduce \emph{rounded interval arithmetic}.

Consider a floating point number $x$ that is given to our algorithm as input; its value is considered exact, and we represent it internally as the singleton $\{x\} = [x,x] \in \intset{\reals}$. When we perform a floating point operation on $x$, the result is %
rounded to fit the precision, if necessary; we know not whether this rounding is up or down, but we know that the exact result lies between two consecutive floating point values.
Therefore, if the \emph{lower} end of the result is computed rounding \emph{down} and the \emph{upper} end is computed rounding \emph{up}, then we know that the true value lies in the interval, even in the presence of rounding.

On a computer, this outward rounding is achieved by internally storing the lower end of the interval with opposite sign, and changing the processor rounding mode to rounding up. This ensures that the interval's width increases only when the actual floating point computation would be inexact. In our code we use the implementation of Attene \cite{attene_indirect_2020}.

When working with intervals as in Algorithm \ref{alg:bisection}, we can use rounded interval arithmetic when evaluating the boxes to guarantee robustness with respect to floating point computations: one gets looser inclusion functions that account for roundoff error.

\subsection{Traversal policy}
\label{sec:traversal}
When an element is valid, the order in which intervals are evaluated is irrelevant, because the whole bisection tree must be visited regardless. By contrast, for invalid elements we wish to confirm the presence of a negative value as soon as possible, so we would like to focus on the most promising areas, i.e. we want to traverse the graph depth-first. Going depth-first has the additional advantage that the number of elements in the data structure $S$ grows linearly with depth (with a factor of $2^n$), whereas for breadth-first search the worst-case space complexity is exponential in depth (with base $2^n$).

When we decide on exploring the graph depth-first, there is still ambiguity on how the children of a node (i.e. sub-boxes) are ordered.
As previously mentioned, we want to explore first the region where it seems most likely that we will find an instance of invalidity. Thus we evaluate each box before adding them to the queue for splitting, and use the result $I\in\intset{\reals}$ of the (minimum) inclusion to prioritize.
We experiment with several priority heuristics: the lower endpoint of $I$, the upper one, or their sum (that is equivalent to using the middle point of $I$).

In this ``guided'' depth-first search, smaller boxes are always processed first. We can relax this constraint and trust the priority estimate more using a priority queue for $S$; however, care must be taken not to explode the search tree as in breadth-first search.
\FS{We can be more specific on this once we are done with the experiments.}

\DP{Results}



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{pictures/positive-jacobian-dataset}
    \caption{Examples of simulation data in 3D. Dirichlet boundary conditions are enforced on the surface of the blue part (top and bottom 20\%), while the yellow part (middle 60\%) is free to move. The model is compressed and twisted at the same time, simulated with \cite{Li2020IPC}.}
    \label{fig:dataset}
\end{figure}

- Baseline newton
- GMSH? not for now


==> bisectionAlgorithm.tex <==
\begin{algorithm}[htb]
	\caption{Element validity with bisection}\label{alg:bisection}
	\begin{algorithmic}[1]
	\Require Elements $e\in\mathcal{M}$ with reference elements $\sigma_e$, Jacobians $J_e$, and minimum inclusion functions $\minclusion{J_e}$; maximum number of iterations $c_{\max}$.
	\Ensure Validity of $\mathcal{M}$: one of \EValid, \EInvalid, \EUncertain.

	\Function{$\prec$}{$(e, B), (e', B')$}
		\Comment{priority function}
		\State \Return \Call{High}{$\minclusion{J_e}{B}$}$<$\Call{High}{$\minclusion{J_{e'}}{B'}$}
	\EndFunction

	\State $S\gets$\Call{PriorityQueue}{$\prec$}
	\Comment{create priority queue for boxes}

	\ForAll{$e\in \mathcal{M}$}
		\State \Call{Push}{$S, (e, [0,1]^{n+1})$}
	\EndFor
	
	\State $c \gets 0$
	\Comment{evaluation counter}
	\While{$\lnot$\Call{IsEmpty}{$S$}}
		\If{$c\geq c_{\max}$}
			\Return{\EUncertain}
			\Comment{give up}
		\EndIf
		\State $c\gets c+1$
		\Comment{increment iteration count}

		\State $(e',B_0) \gets$\Call{Pop}{$Q$}
		\Comment{get the next box from $S$}

		\State $I\gets$\Call{$\minclusion{J_{e'}}$}{$B_0$}
		\Comment{check inclusion}

		\If{\Call{High}{$I$} $\leq 0$}
			\Return{\EInvalid}
			\Comment{element $e'$ is invalid}
		\EndIf

		\If{\Call{Low}{$I$} < 0}
			\Continue{}
			\Comment{element $e'$ is valid}
		\EndIf
		\State $B\gets$\Call{Split}{$B_0$}
		\Comment{split the box in $2^n$ sub-boxes}
		\For{$i \in \{1,\dots,2^n\}$}
			\Comment{for each sub-box}
			\If{$B_i\cap\sigma_{e'}\neq\emptyset$}
				\Comment{$B_i$ intersects reference el.}
				\State \Call{Push}{$S,(e', B_i)$}
					\Comment{push $B_i$ to $S$}
			\EndIf
		\EndFor
	\EndWhile
	\State \Return{\EValid}
	\Comment{all elements are confirmed valid}
	\end{algorithmic}
\end{algorithm}


==> comments.tex <==

\newcommand{\ZH}[1]{}
\newcommand{\EP}[1]{}{}
\newcommand{\DP}[1]{}
\newcommand{\MA}[1]{}
\newcommand{\FS}[1]{}
\newcommand{\fix}[1]{}
\newcommand{\correction}[1]{}


==> formulation_old.tex <==
\section{General framework of element validity}\label{sec:formulation}
Let $n\in\nats$ be the dimension of the embedding space (we may assume $n\in\{2,3,4\}$). We wish to detect invalid $n$-dimensional elements in $\reals^n$.

For each type of element in the mesh, we need to define a common \emph{reference element} $\sigma\subset[0,1]^n$ to act as the coordinate domain for elements of that type. We can use a general description that accounts for all commonly used FEM elements such as triangles, quadrilaterals, tetrahedra, hexahedra, pyramids and prisms.
\begin{definition}[Reference Element]
	Let $s=(*_1,\dots,*_{n-1})$ be a $(n-1)$-tuple of binary operators in $\{+,\max(\cdot,\cdot)\}$. Then the $n$-dimensional reference element $\sigma_s\subset\reals^n$ is defined by the $n+1$ inequalities:
	\begin{gather}
		X_i \geq 0 \quad \forall i=1 \dots n, \\
		(\dots((X_1 *_1 X_2) *_2 X_3)*_3 \dots *_n X_n) \leq 1. \label{eq:ref_ineq}
	\end{gather}
	Call the tuple $s$ the \emph{signature} of the element; in this context, denote the $+$ operator as $\triangle$ and the $\max$ operator as $\square$.
\end{definition}

With this notation we have a general parameter space that works for all the aforementioned types of elements. The 2D standard simplex, normally defined as $\{(x,y)\in\reals^2\mid x\geq0, y\geq0, x+y\leq 1\}$ is the reference element with signature $(\triangle)$; the unit square $[0,1]^2$ can be defined as $\{(x,y)\in\reals^2\mid x\geq0, y\geq0, \max(x,y)\leq 1\}$, and has signature $(\square)$; tetrahedra are $(\triangle, \triangle)$, hexahedra are $(\square, \square)$, pyramids are $(\square,\triangle)$ and wedges or prisms are $(\triangle,\square)$.

To give some geometric intuition on this notation: start from a $1$-dimensional element, i.e. the segment $[0,1]$; each symbol adds a new axis; a $\triangle$ inserts a vertex on the new axis at coordinate $1$ and connects each vertex in the element to the new one; a $\square$ creates a copy of the current element at coordinate $1$ on the new axis, and connects corresponding vertices.

Given an $n$-dimensional reference element $\sigma_s$ and a degree $p\in\nats$, we define the control net of the \emph{uniform} degree $p$ element $\sigma_s^p$ as
\begin{equation}
	\Xi := (1/p)\ints^n \cap \sigma_s
\end{equation}

We can then define a geometric map via the degree-$p$ Lagrange basis polynomials defined for the element $\sigma_s$, with the property that for each point $\xi_i\in\Xi$, $\lagrange{i}(\xi_i)=1$ and $\lagrange{i}(\xi_j)=0$ for any $j\neq i$.

\FS{Explicit definition of $\lagrange{i}$?}

\begin{definition}[Geometric map]
	The (polynomial) geometric map that maps $\sigma_s$ into the physical element $x(\sigma_s)$ is given as:
	\begin{equation}
		x:\sigma_s\to\reals^n \qquad
		x(\xi) := \sum_{\xi_i\in\Xi} x_i \lagrange{i}(\xi_i).
	\end{equation}
	If $\sigma_s$ is uniform of degree $p$, the geometric map is a polynomial map of degree $P:=p(1+s_\square)$, where $s_\square$ is the number of $\square$ symbols in $s$.
\end{definition}
\FS{Review the following claim}
The determinant of the Jacobian matrix $|J_x(\xi)|$ is a polynomial of degree at most $D:=n(P-1)$.
Given a set of control points $\Xi$, our objective is to determine whether the Jacobian $|J_x(\xi)|$ is everywhere greater than 0 on $\sigma_s\subset\reals^n$ or not.

\DP{Instatiate this for P2, Q2, Prism, Pyramid}


\subsection{Time-dependent validity}\label{sec:timedep}
\begin{figure}
	\centering
	\input{timedep.tex}
	\caption{A 2D linear element with linear trajectories that flips twice in a time step, resulting in an element that is valid at both time steps, but invalid in the transition. The element's Jacobian is a polynomial of degree $2$ in $t$ with two distinct real roots.}
	\label{fig:fliptwice1}
\end{figure}

We also consider an extension of the problem that has not been addressed in the previous literature, to the best of our knowledge.
When considering a dynamic simulation, the elements of the mesh move and deform over time. 
Like space, time is approximated by discrete time steps, which are typically regular.
It is customary to approximate the evolution of each element by assuming that its control points move along straight-line trajectories at each time step.
Under these assumptions, we observe that a mesh element may be valid at two consecutive time steps while becoming invalid \emph{in the transition} between them.
Figure \ref{fig:fliptwice1} shows how this transient invalidity can happen even with a linear element in dimension 2. %

We model the time-dependent validity problem as a special case of standard element validity in one additional dimension.
Given any $n$-dimensional reference element $\sigma_s$, the $(n+1)$-dimensional time-dependent version $\sigma_{s\square}$ of that element is constructed by simply appending $\square$ at the end of the signature $s$.
Next, we must define a polynomial on $\sigma_{s\square}$. 
Assuming linear trajectories %
at a constant speed, the $(n+1)$-dimensional element is described by the control net $\{\xi_i^0, \xi_i^1 \mid i\in\Xi\}$, and the geometric map:

\begin{multline}
    x:\reals^{n+1}\to\reals^{n+1} \qquad x(\xi,t) :=
	\sum_{i\in\Xi} ((1-t)x_i^0 + tx_i^1) \lagrange{i}(\xi) = \\
	x(\xi,0) + t(x(\xi,1)-x(\xi,0))
\label{eq:time-dependent}
\end{multline}

where $x(\xi,0)$ and $x(\xi,1)$ are the $n$-dimensional geometric maps of the elements at the two consecutive time steps. We can thus compute the Jacobian determinant as before to obtain a polynomial in $n+1$ variables of degree $nP$, as the variable $t$ only appears with exponent $1$.
Finally, we check its positivity on $\sigma_{s\square}$ using our method.
Note that a more sophisticated evaluation could be assumed, by using splines to model smooth trajectories of the control points; in that case, Equation \ref{eq:time-dependent}, hence its Jacobian, would be of higher degree and impact performance.


Table \ref{tab:degrees} lists the values of $\deg(|J_x|)$ for the most common element types and orders.

\begin{table}
	\begin{tabular}{|l|c|c|c|}
		\hline
		Element name & Symbol & Static & Dynamic \\
		\hline\hline
		Linear triangle & $\sigma_{\triangle}^1$ & 0 & 2 \\
		Quadratic triangle & $\sigma_{\triangle}^2$ & 2 & 4 \\
		Cubic triangle & $\sigma_{\triangle}^3$ & 4 & 6 \\
		Quartic triangle & $\sigma_{\triangle}^4$ & 6 & 8 \\
		Quintic triangle & $\sigma_{\triangle}^5$ & 8 & 10 \\
		\hline
		Bilinear quadrangle & $\sigma_{\square}^1$ & 1 & 4 \\
		Biquadratic quadrangle & $\sigma_{\square}^2$ & 6 & 8 \\
		Bicubic quadrangle & $\sigma_{\square}^3$ & 10 & 12 \\
		\hline\hline
		Linear tetrahedron & $\sigma_{\triangle\triangle}^1$ & 0 & 3 \\
		Quadratic tetrahedron & $\sigma_{\triangle\triangle}^2$ & 3 & 6 \\
		Cubic tetrahedron & $\sigma_{\triangle\triangle}^3$ & 6 & 9 \\
		Quartic tetrahedron & $\sigma_{\triangle\triangle}^4$ & 9 & 12 \\
		\hline
		Bilinear tri. prism & $\sigma_{\triangle\square}^1$ & 3 & 6 \\
		\hline
		Trilinear hexahedron & $\sigma_{\square\square}^1$ & 6 & 9 \\
		Triquadratic hexahedron & $\sigma_{\square\square}^2$ & 15 & 18 \\
		\hline
	\end{tabular}
	\caption{Maximum degree of the Jacobian determinant polynomial.}
	\label{tab:degrees}
\end{table}


==> grid.tex <==
\section{Grid search}
Let $r\in\nats$. We define
\begin{equation}
	\Delta^n(r) := \{x\in\Delta^n \mid rx \in \ints^{n+1}\}
\end{equation}
the set of rational points of $\Delta^n$ with denominator $r$.
Denote $f_{\min}^{\Delta^n(r)}$ the minimum of $f$ on ${\Delta^n(r)}$.
Obviously, as $\Delta^n(r)\subset \Delta^n(2r)$, $f_{\min}^{\Delta^n(r)}\geq f_{\min}^{\Delta^n(2r)}\geq f_{\min}$.


Given $y\in\reals^{n+1}$, define its \emph{support} as:
\begin{equation}
	\support(y) := \{i \in \{0,\dots,n\} \mid y_i \neq 0\}.
\end{equation}
The following convergence result is proven in \cite{de_klerk_convergence_2017}.
\begin{theorem}\label{thm:ogbound}
	Consider a polynomial $f(X)=\sum_{|\alpha|\leq D}f_\alpha X^\alpha$ of degree $D$.
	Then for all positive integers $r$:
	\begin{equation}
		f_{\min}^{\Delta^n(r)} - f_{\min} \leq \frac{C_f}{r^2}
	\end{equation}
	where $C_f\in\reals$ is
	\begin{equation}
		C_f := \frac{D(D-1)}{2}\left(1-\frac{1}{|\support(f_{\min})|}\right)^2 \sum_{|\alpha| \leq D} |f_\alpha|.
	\end{equation}
\end{theorem}
This theorem tells us that, given $r\in\nats$, $f_{\min}$ is bounded by $f_{\min}^{\Delta^n(r)}$ from above and by $f_{\min}^{\Delta^n(r)} - C_f/r^2$ from below.

Since we do not know the support of $f_{\min}$ (i.e. we do not know whether the minimum lies within the interior of the simplex or on a facet), we have to assume the worst case where $|\support{f_{\min}}|=n+1$. So we must re-define $C_f$ to be
\begin{equation}
	C_f := \frac{D(D-1)}{2}\left(\frac{n}{n+1}\right)^2 \sum_{|\alpha| \leq D} |f_\alpha|
\end{equation}
which is greater than the original value.


\begin{algorithm}[htb]
	\caption{Element validity with grid search}\label{alg:valid}
	\begin{algorithmic}[1]
	\Require Polynomial Jacobian determinant $f = |J_x(X)|$.
	\Ensure Validity of the element: one of \EValid, \EInvalid, \EUncertain.

	\State Compute the constant $C_f$
	\State $r\gets 1$
	\Comment {refinement level of the grid}
	\State $Q\gets $\Call{Queue}{$\Delta^n(1)$}
	\Comment{queue of points to evaluate}
	\State $\mu\gets f($\Call{Pop}{$Q$}$)$
	\Comment {minimum of samples evaluated so far}
	\Repeat
		\If{$\mu\leq 0$}
			\Return \EInvalid
			\Comment{element is invalid}
			\EndIf

		\If{$Q=\varnothing$}
			\Comment{when the whole level $r$ has been evaluated}
			\If{$r^2 \mu>C_f$}
			\Return \EValid
			\Comment{element is valid}
			\EndIf
			\State $Q\gets \Delta^n(2r)\setminus\Delta^n(r)$
			\Comment{push points not already evaluated to queue}
			\State $r\gets 2r$
			\Comment{double the refinement level}
		\EndIf

        \State $\mu\gets \min\{\mu, f($\Call{Pop}{$Q$}$)\}$
		\Comment{check next point and update minimum}
	\Until{$r>r_{\max}$}
    \Return \EUncertain
	\Comment{after $r_{\max}$ refinements we give up}
	\end{algorithmic}
\end{algorithm}

We can thus use Algorithm \refeq{alg:valid} to determine the validity of mesh elements. In the algorithm we sample the simplex one point at a time, making sure we don't find points with negative values; when we run out of points to check for a level, we check if the bound is enough to guarantee positivity everywhere, and if not we double the grid resolution and continue. We also set a maximum number of iterations $r>r_{\max}$.

Algorithm \refeq{alg:valid} has quadratic order of convergence, like the one in \cite{johnen_geometrical_2014}.




\subsection{Tightening the lower bound}
The coefficient $C_f$ is computed only once per element and it determines how fast the grid search algorithm converges. Therefore, we would like it to be as small as possible: we now prove a bound for monomials defined on the simplex that can be used to improve $C_f$.

The number $D(D-1) \sum_{|\alpha| \leq D} |f_\alpha|$ in the formula for $C_f$ is the factor that we want to attack. It comes from the following lemma that appears in the proof of Theorem \refeq{thm:ogbound}:
\begin{lemma}\label{lem:secder}
	Consider a polynomial $f(X)=\sum_{|\alpha|\leq D}f_\alpha X^\alpha$ of degree $D$.
	Then for any point $y \in [0,1]^{n+1}$:
	\begin{equation}
		\sum_{i,j=0}^n |\nabla^2f(y)_{i,j}| \leq D(D-1)\sum_{|\alpha| \leq D}|f_\alpha|.
	\end{equation}
\end{lemma}
As we only care about points in $\Delta^n\subsetneq[0,1]^{n+1}$, we can put a tighter upper bound on $\sum_{i,j=0}^n |\nabla^2f(y)_{i,j}|$.
Let us begin by proving an intermediate result.

\begin{lemma}\label{lem:maximum}
	Let $\alpha\in\nats^{n+1}$, and $x_\alpha := (\alpha_i/|\alpha|)_{i=0}^n \in \Delta^n$. The maximum of the monomial function $X^\alpha$, restricted to $\Delta^n$, is 
	\begin{equation}
		M(\alpha):=(x_\alpha)^\alpha=\frac{1}{|\alpha|^{|\alpha|}} \prod_{\substack{i=0 \\ \alpha_i\neq 0}}^n \alpha_i^{\alpha_i} \in \reals.
	\end{equation}
\end{lemma}
\begin{proof}
	Denote with $e_i$ the $i$-th column of the $(n+1)\times(n+1)$ identity matrix, and define $e:=\sum_{i=0}^n e_i$.

	First of all, observe that $X^\alpha$ is continuous and $\Delta^n$ is compact, so a global maximum always exists.

	We first consider the case where $\alpha_i \neq 0$ for all $i=0,\dots,n$.
	Define $h(X):= 1-\sum_{i=0}^n X_i$;
	by the theorem of Lagrange multipliers, if $y\in\reals^{n+1}$ is an extremum of $X^\alpha$ constrained by $h(X)=0$, then $\nabla X^\alpha$ is parallel to $\nabla h = -e$, which means that all entries of $(\nabla X^\alpha)^\top = (\alpha_i X^{\alpha-e_i})_{i=0}^n$ are equal.
	For all pairs $j,k\in \{0,\dots,n\}$, we have that
	\begin{align}
		&\alpha_j X^{\alpha-e_j}=\alpha_k X^{\alpha-e_k} \\
		\implies& \alpha_j X^{\alpha+e_k}=\alpha_k X^{\alpha+e_j} \\
		\implies& \alpha_j X_k = \alpha_i X_j \\
		\implies& \frac{X_j}{\alpha_j} = \frac{X_k}{\alpha_k},
	\end{align}
	so if $y$ is a local extremum then $y_i/\alpha_i$ is equal to a constant $\lambda \in \reals$ for all $i$, and $h(y)=0$.
	The first condition implies that $y^\top = (\alpha_i \lambda)_{i=0}^n$; the second condition gives $\lambda=1/|\alpha|$.
	Hence, we have that $y=x_\alpha$ is the only local extremum of $X^\alpha$ restricted to the hyperplane defined by $h(X)=0$, and therefore $x_\alpha$ is the only local extremum of $X^\alpha$ on $\Delta^n$.
	Obviously, since we assumed that $\alpha_i\neq 0$ for all $i$, we have $0<X^\alpha\leq 1$ in the interior of $\Delta^n$ and $X^\alpha \equiv 0$ on the boundary, so the maximum must lie in the interior of $\Delta^n$. Because the only local extremum in $\Delta^n$ is $x_\alpha$, which is not on the boundary, $x_\alpha$ must be the global maximum.


	Now we describe the case with $\alpha_i=0$ for some $i$.
	Observe that for $I\subsetneq\{0,\dots,n\}$, $q:=n-|I|$, the set $\Delta_I:=\{x \in \Delta^n | x_i = 0 \, \forall i \in I\}\subset\Delta^n$ is a $q$-dimensional facet of the $n$-simplex $\Delta^n$. By projection $\pi$ on the $q+1$ coordinates whose indices are not in $I$, we have $\pi(\Delta_I)=\Delta^q\subset\reals^{q+1}$; moreover, $\pi(X^\alpha)$ is defined on $\Delta^q$, and $X^\alpha|_{\Delta_I}\equiv\pi(X^\alpha)$.

	Given $y\in\Delta^n$, consider $z\in\Delta_I$ a point with the property that $z_i=0$ for all $i$ such that $\alpha_i=0$, and $z_i\geq y_i$ otherwise.
	It is clear that $z^\alpha\geq y^\alpha$ by construction, therefore the global maximum must lie in $\Delta_I$.
	The maximum of $X^\alpha$ on $\Delta^n$ is therefore equal to the maximum of $\pi(X^\alpha) = \pi(X)^{\pi(\alpha)}$ on $\Delta^q$; by construction, $\pi(\alpha)$ has no zero components, so we can apply the same argument we used in the case $\alpha_i\neq 0$ for all $i$, only in dimension $q<n$, to conclude.
\end{proof}


\begin{lemma}[Tightened Lemma \refeq{lem:secder}]\label{lem:newsecder}
	Consider a polynomial $f(X)=\sum_{|\alpha|\leq D}f_\alpha X^\alpha$ of degree $D$.
	Then for any point $y \in \Delta^{n+1}$:
	\begin{equation}
		\sum_{i,j=0}^n |\nabla^2f(y)_{i,j}| \leq \sum_{|\alpha|\leq D} |f_\alpha| B(\alpha)
	\end{equation}
	where
	\begin{equation}
		B(\alpha) :=
			\sum_{i,j=0}^n \alpha_i \alpha_j M(\alpha-e_i-e_j) - \sum_{i=0}^n \alpha_i M(\alpha-2e_i).
	\end{equation}
	Moreover, this bound is tighter than the one in Lemma \refeq{lem:secder}.
\end{lemma}
\begin{proof}
	Following the proof of Lemma \refeq{lem:secder}, we compute
	\begin{equation}
		\nabla^2f(y)_{i,j} = \begin{cases}
			\sum_{|\alpha|\leq D} f_\alpha \alpha_i \alpha_j y^{\alpha-e_i-e_j} & i\neq j \\
			\sum_{|\alpha|\leq D} f_\alpha \alpha_i (\alpha_i-1) y^{\alpha-2e_i} & i = j
		\end{cases}.
	\end{equation}
	By summing over $i,j$ we obtain
	\begin{align}
		\sum_{i,j=0}^n &|\nabla^2f(y)_{i,j}| \\
		&\leq \sum_{\substack{i,j=0\\i\neq j}}^n \sum_{|\alpha|\leq D} |f_\alpha| \alpha_i \alpha_j y^{\alpha-e_i-e_j} + \sum_{i=0}^n \sum_{|\alpha|\leq D} |f_\alpha| \alpha_i (\alpha_i-1) y^{\alpha-2e_i} \\
		&\leq \sum_{|\alpha|\leq D} |f_\alpha| \left(\sum_{\substack{i,j=0\\i\neq j}}^n \alpha_i \alpha_j M(\alpha-e_i-e_j) + \sum_{i=0}^n \alpha_i (\alpha_i-1) M(\alpha-2e_i)\right) \\
		&= \sum_{|\alpha|\leq D} |f_\alpha| \left(\sum_{i,j=0}^n \alpha_i \alpha_j M(\alpha-e_i-e_j) - \sum_{i=0}^n \alpha_i M(\alpha-2e_i)\right) \\
		&= \sum_{|\alpha|\leq D} |f_\alpha| B(\alpha).
	\end{align}
	To prove that this bound is better than the one in Lemma \refeq{lem:secder} we simply finish the proof as in \cite{de_klerk_convergence_2017}:
	\begin{align}
		\sum_{|\alpha|\leq D} |f_\alpha| B(\alpha)
		&\leq \sum_{|\alpha|\leq D} |f_\alpha| \left(\sum_{i,j=0}^n \alpha_i \alpha_j - \sum_{i=0}^n \alpha_i\right) \\
		&= \sum_{|\alpha|\leq D} |f_\alpha| \left(\left(\sum_{i=0}^n \alpha_i\right)^2 - \sum_{i=0}^n \alpha_i\right) \\
		&\leq D(D-1) \sum_{|\alpha|\leq D} |f_\alpha|.
	\end{align}
\end{proof}
Notice that $B(\alpha)$ does not depend on $f$ and as such can be pre-computed and reused across elements.
We can also write it as
\begin{equation}
	B(\alpha) = \sum_{i=0}^n \alpha_i \left( \sum_{j=0}^n\alpha_j M(\alpha-e_i-e_j) - M(\alpha-2e_i) \right)
\end{equation}

We can use this result to prove the following:
\begin{theorem}\label{thm:newbound}
	Consider a polynomial $f(X)=\sum_{|\alpha|\leq D}f_\alpha X^\alpha$ of degree $D$.
	Then for all positive integers $r$:
	\begin{equation}
		f_{\min}^{\Delta^n(r)} - f_{\min} \leq \frac{C_f}{r^2}
	\end{equation}
	where $C_f\in\reals$ is
	\begin{equation}
		C_f := \frac{1}{2}\left(\frac{n}{n+1}\right)^2 \sum_{|\alpha| \leq D} |f_\alpha| B(\alpha).
	\end{equation}
\end{theorem}
\begin{proof}
	Identical to the proof of Theorem \refeq{thm:ogbound}, but using Lemma \refeq{lem:newsecder} instead of Lemma \refeq{lem:secder}.
\end{proof}

We can plug this new $C_f$ right into Algorithm \refeq{alg:valid}. This makes convergence much faster, but the algorithm is still not adaptive.











==> quadrature.tex <==
\section{Inversion-aware quadrature}
\label{sec:quadrature}


==> table-exp-old.tex <==
\begin{table*}
	\begin{tabular}{l|l|cc|c|r|r|r|r|r|r|r|r|r}
		Dataset & Element & $n$ & $s$ & $p$ & \multicolumn{3}{c|}{\# elements} & \multicolumn{6}{c}{time per element ($\mu$s)}\\
            & & & & & tot & valid & invalid & pre & avg & valid & invalid & max & std \\
		\hline
            Kangaroo & Triangles & 2 & 2 & 1 & 172800 & 146248  & 26552 & 9   & 3   & 1   & 21  & 29  & 4\\
                     && & & 2 & 172800 & 145602  & 27198 & 12  & 12  & 9   & 28  & 189   & 7\\
                     && & & 3 & 172800 & 145623  & 27177 & 33  & 52  & 47  & 80  & 295   & 12\\
                     && & & 4 & 172800 & 118436 & 27187 & 89 & 187 & 177 & 240 & 1035 & 24\\
            Bar & Quadrangles & 2 & 1 & 1 & 130291 & 130244  & 47 & 16   & 8   & 8   & 21  & 73  & 1\\
                     && & & 2 & 31879 & 31808  & 71 & 115   & 125   & 125   & 348  & 2021  & 22\\
            Armadillo & Tetrahedra & 3 & 3 & 1 & 54985 & 51605 & 3380 & 21 & 2 & 1 & 9 & 19 & 2\\
                     && & & 2 & 54985 & 48599 & 6386 & 229 & 280 & 268 & 373 & 24197 & 142\\
                     && & & 3 & 54985 & 47988 & 6997 & 1936 & 4720 & 4216 & 8173 & 176461 & 3357\\
            Bunny & Tetrahedra & 3 & 3 & 1 & 19800 & 19561 & 239 & 24 & 1 & 1 & 10 & 69 & 1\\
                    && & & 2 & 19800 & 19058 & 742 & 235 & 277 & 270 & 451 & 7132 & 98\\
                     && & & 3 & 19800 & 18954 & 846 & 1964 & 4290 & 4133 & 7811 & 84298 & 1731\\
	\end{tabular}
	\caption{Results of our continuous validity test on simplicial datasets of dimension $n=2$ (Kangaroo) and $n=3$ (Armadillo and Bunny), and a tensor product dataset of dimension $n=2$ (Bar), with elements of various order $p$. We report the number of elements (total, valid on the whole interval, elements with a shorter validity time) and time per element for the processing (pre-processing, average, average per valid elements, average per invalid elements, maximum, standard deviation).}
	\label{tab:exp}
\end{table*}


==> timetable.tex <==
\begin{tabular}{cc|r|r|rrr}

$n$ & $p$ & Method & Avg. $\mu$s & \textsc{FV} & \textsc{FI} & \textsc{U} \\ \hline 

\multirow{2}{*}{2} & \multirow{2}{*}{2} & Naive & 3.35 & 85 & 0 & 0 \\
& & Bisection & 3.93 & 0 & 0 & 0 \\ \hline 

\multirow{2}{*}{2} & \multirow{2}{*}{3} & Naive & 5.26 & 55 & 0 & 0 \\
& & Bisection & 6.43 & 0 & 0 & 0 \\ \hline 

\multirow{2}{*}{2} & \multirow{2}{*}{4} & Naive & 10.37 & 45 & 0 & 0 \\
& & Bisection & 11.79 & 0 & 0 & 0 \\ \hline 

\multirow{2}{*}{2} & \multirow{2}{*}{5} & Naive & 19.25 & 11 & 0 & 0 \\
& & Bisection & 3245.18 & 0 & 0 & 0 \\ \hline 

\multirow{2}{*}{3} & \multirow{2}{*}{2} & Naive & 12.06 & 1543 & 0 & 0 \\
& & Bisection & 28.70 & 0 & 0 & 0 \\ \hline 

\end{tabular}

